DSIC: Deep Stereo Image Compression

In this paper we tackle the problem of stereo image compression, and leverage the fact that the two images have overlapping fields of view to further compress the representations. Our approach leverages state-of-the-art single-image compression autoencoders and enhances the compression with novel parametric skip functions to feed fully differentiable, disparity-warped features at all levels to the encoder/decoder of the second image. Moreover, we model the probabilistic dependence between the image codes using a conditional entropy model. Our experiments show an impressive 30 - 50% reduction in the second image bitrate at low bitrates compared to deep single-image compression, and a 10 - 20% reduction at higher bitrates.

==> approach.tex <==
% !TEX root = top.tex
% In section: Approach
\section{Deep Stereo Compression}

\begin{figure*}[t]
	\centering
	\includegraphics[width=1.\linewidth]{figures/stereo_complex_model.pdf}
	\caption{An iIlustration of the volumetric disparity skip functions. \slwang{let's talk about the figure on Monday}}
	\label{fig:stereo_complex_model}
\end{figure*}


%\raquel{not clear to me that we want to write paper as stereo, or as cameras that have overlapping fields of view, and thus is more general. Then we demonstrate this in the stereo case}

In this paper we tackle the problem of compressing a pair of stereo images. % that have overlapping fields of view. 
%\shenlong{Specifically, we focus on compressing a pair of stereo images.}
%Our intuition is that since these cameras see the same scene, by compressing them jointly we can further save in storage. 
Intuitively, if the overlapping field of view 
between the stereo  pair 
is very high, then the bitrate of the combined latent code should be lower than the sum of the bitrates if we compressed the images separately; at the very least it cannot be higher. 

More formally, let us denote $\jmb{x}_1, \jmb{x}_2$ as a pair of rectified stereo images and let $H(\jmb{x}_1, \jmb{x}_2)$ be the entropy of the stereo pair.  Given the fact that a stereo pair sees the same scene with difference up to a small camera pose offset, $\jmb{x}_1$ and $\jmb{x}_2$ are dependent on each other. \raquel{correlated instead of dependent on each other?}
%We denote the entropy of the stereo pair as $H(\jmb{x}_1, \jmb{x}_2)$. 
According to information theory, 
%we denote the entropy of the stereo pair as $H(\jmb{x}_1, \jmb{x}_2)$, 
then there should exist a margin between the joint entropy $H(\jmb{x}_1, \jmb{x}_2)$ and the sum of individual ones $H(\jmb{x}_1) + H(\jmb{x}_2)$. In other words, the mutual information $I(\jmb{x}_1, \jmb{x}_2) = H(\jmb{x}_1) + H(\jmb{x}_2) - H(\jmb{x}_1, \jmb{x}_2) > 0$. 
% \slwang{
%% We haven't formally define $x_1$ and $x_2$. 
%Make sure to use bold for vectors/multivariate variables in the whole paper.}
%\jerry{I don't want to suggest that the MI has to be large because it would lead the reviewers to expect that we would extract bigger gains than what we have} 

This observation motivates our general approach: we propose a single compression model that jointly compresses two stero images. Towards this goal, we focus on extracting as much information as possible from one image (the "reference" image) in order to reduce the bitrate in the second (the "residual" image), such that the joint bitrate is lower than the result of independent single-image compression. Our approach consists of two main components: adding \textit{multi-level skip functions} from the first image feature maps such that \raquel{say why this makes sense}, as well as learning a \textit{conditional entropy model}. Our skip functions help to improve reconstruction quality for a given bitrate by extracting information
from the feature maps of the first image, while our conditional entropy model models the inherent dependence of the residual code with the reference code. 
\raquel{rewrite the paragraph to explain one after another, instead of first saying both and then explaining. Its easier to read}
The two components are based on the following facts respectively: 1) features from a stereo pair are more related if we warp one with a good disparity estimation; 2) the codes of two images are dependent given the dependence of the input. \raquel{this hould be pass at the begining of this paragraph where you give context avbout the two components not at the end.}

%\shenlong{The two components based on the following facts respectively: 1) features from a stereo pair are more related if we warp one with a good disparity estimation; 2) the codes of two images are dependent given the dependence of the input.}  
%\slwang{the sentence above is a bit too vague here. Jerry could you rephrase better?}
%\raquel{add one sentence intuition of what these two things are}
%\slwang{We should move some of the content to intro. Let's decide when do an intro pass.}
%\jerry{I'm actually not sure how to make this more specific, I don't think mentioning "good" disparity estimation is good because we don't necessarily learn "good" disparity estimates with our disparity volumes.}


%our work can be seen as an extension that can be applied on top of existing single-image autoencoder architectures for compression. We start with a single-image architecture model and try modeling relationships between images to reduce the joint entropy. 

\subsection{Overview} 
% To start, assume we are given a rectified stereo image pair $x_1, x_2$. 
% \slwang{already defined}
Our stereo compression architecture consists of a pair of autoencoders, each consisting of an encoder, quantizer, and decoder. We  denote each encoder/quantizer/decoder as $E_1, Q_1, D_1$ and $E_2,Q_2,D_2$ respectively, where $E_i,Q_i,D_i$ are used to encode/decode $\jmb{x}_i$. 
% \raquel{also we might want to write this in the multiimage setting, not just in the 2 camera setting.} \slwang{resolved after discussion}
As shown in  Fig. \ref{fig:stereo_complex_model}, there exist connections from the feature maps of $E_1$ to $E_2$ and $D_1$ to $D_2$, which we will denote as \textit{skip functions}; these skip functions provide the mechanism of passing information from $\jmb{x}_1$ to help with the encoding/decoding of $\jmb{x}_2$. We provide more details below: Section \ref{sec:feature_map} will discuss the encoder/decoder layers and quantization mechanism, Section \ref{sec:vol_disparity} discusses the nature of these skip functions, and Section \ref{sec:entropy_model} discusses our entropy model. 

\raquel{this section is not really providing anything wrt the text above...  instead Ill pass this to before "overview", and only the sentence about we now... The definition of E, Q, P can go to what is now 3.2 and start with this.}

%\slwang{Notations are still not very good. Could you make sure you address my comments by changing vectors with bold font?}

\subsection{Feature Encoding/Decoding and Quantization} \label{sec:feature_map}
Our encoder, decoder, and quantizer pair \raquel{its a trio, not pair ;)} borrow their architectures from the factorized prior single-image compression model in Balle et al. \cite{balle_varhyperprior}.  The encoder is implemented with a series of 4 downsampling convolutions (by 2x) and  Generalized Divisive Normalization (GDN) layers \cite{balle_gdn}. The decoder $D$ is implemented with a series of 4 upsampling deconvolutions (by 2x) and Inverse-GDN layers. During inference, the quantizer $Q$ applies a rounding function to the floating-point output of the encoder $Q(E(\jmb{x})) = Q(\jmb{y}) = \hat{\jmb{y}}$. The dimension of $\hat{\jmb{y}}$ is $M \times H/16 \times W/16$. Similar to \cite{balle_imgcomp_end2end, balle_varhyperprior}, the quantizer applies additive uniform noise during training $Q(\jmb{y}) = \bar{\jmb{y}}$. \raquel{its odd that you are talking about training here, while you havent talk about loss function or anything. Ill pass this to learning subsection}
However, similar to \cite{lee_contextadapt}, we use $\hat{\jmb{y}}$ as the input into the decoder and only use $\bar{\jmb{y}}$ as input into our entropy model (Section \ref{sec:entropy_model}); we found that this yielded a smaller discrepancy in error metrics between training and inference. 
Please refer to the supplementary material for more detailed computation graph of each module. \raquel{this is hard to understand since you havent define anything yet...}
%\slwang{The two equation could not hold true at the same time. Which one is the additive noise? Add the noise explicitly. }


%\subsection{Adding one-sided skip functions for stereo compression} 
% \subsection{Warped skip connection}
\subsection{Volumetric Disparity Warped Skip Functions} \label{sec:vol_disparity}

\raquel{we need a paragraph stating what we are going to see in this section and the intuitions. Its hard to follow for someone that doesnt know what you have done}

\paragraph{General Skip Function Structure:}
In order to ``extract" information from the first image, we can add a ``skip function" $g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma})$ from $D_1$ to $D_2$, where $\jmb{h}^t_1, \jmb{h}^t_2$ are the feature maps in $D_1$ and $D_2$ at a given level $t$, and $\jcb{\gamma}$ is a function of the main image code and incorporates global context information. \raquel{yes we can do that but you need to say why this is a good idea. Give always motivation of your choices to help the reviewer understand why what you did makes sense}
Details for $\jcb{\gamma}$ described at the end of Sec. \ref{sec:vol_disparity}. \raquel{this is odd as this is that section!}
%\slwang{define $\gamma$ more formally / specifically}
Each skip function output is  concatenated with the feature map at $D_2$ before the next upsampling convolution. 
% We denote $g_l$ as a skip function rather than a skip connection because while $g_l$ could be modeled as a traditional skip connection (an identity function $(g_l(h^t_1, h^t_2, \gamma) = h^t_1$, it can be any arbitrary function. 
Note that the skip function is a generalized case of skip connection in residual modules. 
It is degraded to standard skip connections when $g_l$ is an identity function ($g_l(\jmb{h}^t_1, 
\jmb{h}^t_2, \jcb{\gamma}) = \jmb{h}^t_1$). In our experiments, we show that a nonlinear deep warping function increases the flexibility of how information is propagated from one image to the other. \raquel{maybe say form reference image to X image. As current sentence sort of hints symmetry, which is not}
\raquel{we need a fancy name for this skip functions. Parametric skip functions? Or something}
% We denote $g_l$ as a skip function rather than a skip connection because while $g_l$ could be modeled as a traditional skip connection (an identity function $(g_l(h^t_1, h^t_2, \gamma) = h^t_1$, it can be any arbitrary function. 

%Hence the combined skip function, convolution, and activation layer $f_l$ in $D_2$ can be viewed as 
%\begin{equation}
%\begin{aligned} \label{eq:update}
%\jmb{h^{l+1}_2} = f_{l+1}(Conv(Concat(\jmb{h}^t_2, g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}))))
%\end{aligned}
%\end{equation}
%%\slwang{$f$ is not defined.}
%Here, we have presented skip functions in the decoder. 
%% For our stereo compression models, w
%We have similarly implemented skip functions in the encoder as well and found marginally better results. Our skip functions range from levels $l=1,2,3$, where $l=4$ represents the final reconstruction of the image $\hat{\jmb{x}}_1, \hat{\jmb{x}}_2$. Hence, the maximum height/width of $\jmb{h}^t_1$, $\jmb{h}^t_2$ used in $g_l$ is $H/2, W/2$. 

%In the simplest case, we do model $g_l$ as an identity function, so effectively each $h^t_1, h^t_2$ is concatenated into a convolutional layer in $D_2$. This can work to a degree if the baseline between the stereo pair is not too wide and there exists shared information within a few pixels of each other between the two images. We refer to this model as the ``Simplified Stereo Model" (SSM). \slwang{Given complext model has better performance, probably we should move the this paragraph ssm to ablation study instead, showcasing skip function is better than skip connection in our model, instead of proposing two models.}
%\jerry{Removed the SSM paragraph, will put into experiments/ablation.}

%\subsection{Volumetric Disparity-warped skip functions} \label{sec:vol_disparity}

\paragraph{Predicting Volumetric Disparities for Feature Warping:}
In our skip functions, we aim to obtain good disparity estimates between a stereo pair to better warp feature maps between $E_1,D_1$ to $E_2,D_2$. But there are a few caveats and considerations. First, we  designed our skip functions to be present at every feature map resolution. This is due to the fact that  feature maps at each level in $E,D$ contain different layers of high-level and low-level information. Thus  the optimal disparity estimates to warp a feature map at one level in $E_1,D_1$ for $E_2,D_2$ may not be the optimal estimates at another level.

Moreover, as mentioned in Section \ref{sec:related_work}, existing stereo matching networks are inefficient and suboptimal, especially with the absence of ground-truth depth to train the network. \raquel{why are we talking about absence of GT?}
We found that using a separate stereo matching network to predict disparities at each level quickly overstepped GPU memory limits, and that using a single stereo matching network to predict disparities for all resolution levels produced suboptimal results. 

%\slwang{the above two subsections are not well structured. we might want to make some changes, perhaps merge here. } \jerry{Tried to do some rearranging.}


%\begin{figure*}
%	\centering
%	\includegraphics[width=\linewidth]{figures/bilinear_ex.png}
%	\caption{Demonstration of a failure case for bilinear sampling when training disparities on a consistency/photometric loss. Given the green point in camera 2, the plots demonstrate the photometric loss given a disparity (in the leftward x-direction) from the same point in camera 1. The correct disparity (as well as the minimum) is given by the green line, and the predicted disparity is given by the blue dot. The disparity update vector is shown by the blue arrows. In (b), bilinear sampling only provides information on the neighboring pixel values, and so the disparity is pushed further to the right. In (c), the disparity volume (purple region) contains information of all pixels within its range (starting from 0), which contains the ideal minimum, and the gradient pushes the disparity closer to the true value.}
%	\label{fig:bilinear_ex}
%\end{figure*}

In order to use disparities to extract the right feature information at each level, we propose skip functions that predicts and makes use of \textit{volumetric} disparity estimates. Each skip function first outputs a cost volume $\jmb{S}^t = s_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma})$ of dimension $B \times D \times H^t \times W^t$, where $B$ is batch size and $D$ is the disparity range. Each value in the cost volume can be seen as a probability/confidence measure of the correct disparity at that coordinate. Then, if $C^t$ is the channel dimension of $\jmb{h}^t_1$, we also expand $\jmb{h}^t_1$ into a volumetric representation $\jmb{V}^t_1$ of size $B \times C^t \times D \times H^t \times W^t$, where each disparity dimension represents $\jmb{h}^t_1$ offset by disparity $d$. The cost volume is then used to ``select" values from $\jmb{V}^t_1$. This skip function can be represented as the following: 

%\slwang{define B, C, H, W, V otherwise} \jerry{V is defined; H/W are pretty obvious; I'll define B/C}.

\begin{equation}
\begin{aligned} \label{eq:complex_skip}
g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}) = \sum_{d=0}^{D}{\jmb{S}^t_d \cdot
	\jmb{V}^t_{1d}} 
\end{aligned}
\end{equation}
%\slwang{talk about if you ensure the cost is non-negative and if cost is normalized in any form. You haven't talk about $S^t$'s architecture as well} \jerry{Architecture is briefly described in the last paragraph of this section but not sure if it can be moved to supp.}
We apply a softmax across every disparity dimension in $\jmb{S}^t$, so each value represents a probability estimate of disparity $d$ in pixel position $0 \leq i,j \leq W^t, H^t$. 
Our approach of directly using the cost volumes for sampling is similar to those of appearance synthesis papers, such as \cite{xie_deep3d,flynn_deepstereo}, but to our knowledge this is the first time this has been used for compression. Since we regress a separate cost volume at each level $t$, we allow for more flexible spatial relationships amongst the different feature map levels. 

%Finally, we have observed both theoretically and empirically that bilinear sampling, a tool used in stereo matching and depth estimation to sample images in another frame using disparity estimates, is not suitable for learning disparities. Every since \cite{jaderberg_spatialtransform} showed that bilinear sampling was a locally differentiable operation, different papers \cite{godard_leftright, garg_depthest, zhong_selfsupstereo} have used bilinear sampling to learn disparities using photometric loss and left-right consistency loss. However, we observe that bilinear sampling and related sampling kernels by definition do not obtain information beyond the immediately adjacent pixels to the disparity estimates. As a result, it is incredibly difficult for the proper disparity to be learned if the proper disparity falls more than a few pixels beyond the current disparity estimate.
%See Fig. \ref{fig:bilinear_ex} for an illustration of this problem. 
%\slwang{I am a bit worried about this claim since there are quite a few unsupervised learning approach using photometric loss over bilinear sampled warping as supervision. People can easily question here since we don't given enough convincing evidence. I am leaning towards to rephrasing this as that disparity volume warping build connections from more pixels from left image to a target pixel at right than bilinear interpolation. So from architecture perspective not optimization perspectives} 
%\jerry{Commented out the relevant chunk of text - I tried to rewrite this a little bit.}

We also considered directly regressing the disparity estimate from the cost volume, and then using bilinear sampling as in \cite{jaderberg_spatialtransform} to warp the feature maps in a differentiable manner, similar to \cite{zhong_selfsupstereo, godard_leftright, garg_depthest}. However we found that directly using the cost volume for feature selection allowed the model to learn a more flexible weighted arrangement between an entire disparity range of pixels instead of just between two. Also, we empirically observed that since bilinear sampling kernels are only locally differentiable between two adjacent pixels, we found it hard to tune our compression models to learn any meaningful disparities in this manner, even when trained with additional regularization such as smoothness. (TODO: put in supp?) 
%Using a cost volume for sampling instead of regressing a disparity estimate first bypasses the local differentiability problem presented by bilinear sampling kernels. 
\paragraph{Incoporating Global Context for Disparity Prediction}
We've defined $\jmb{S}^t$ as a function of $\jmb{h}^t_1, \jmb{h}^t_2$ and a context term $\jcb{\gamma}$. The goal of $\jcb{\gamma}$ is to incorporate global or external information to better learn $\jmb{S}^t$; we've designed $\jcb{\gamma}$ as $\gamma(\bar{\jmb{y}}_1, l)$, a function of the first image code and the current level.  The output of $\jcb{\gamma}(\bar{\jmb{y}}_1, l)$ is an ``initial disparity volume" $\jmb{S^{\gamma_l}}$ of dimensions $B \times C^{\jcb{\gamma_l}} \times D \times H/16 \times W/16$. By taking in $\bar{\jmb{y}}_1$ as input, $\gamma(\bar{\jmb{y}}_1, l)$ offers our network a view of the global image context - moreover, $\gamma$ provides separate pathways to learn an initial ``monocular" estimate of the disparities at each level, based on $\bar{\jmb{y}}_1$, before being concatenated with $\jmb{h}^t_1, \jmb{h}^t_2$ to predict the final $\jmb{S}^t$. The pathways to predict $\jcb{\gamma}$ from $\bar{\jmb{y}}_1$ and $t$ are solely focused on learning disparities and not reconstruction, unlike those forming $\jmb{h}^t_1, \jmb{h}^t_2$. We could not include $\bar{\jmb{y}}_2$ as an input into $\jcb{\gamma}$ because $\jmb{S}^t$ is used during the encoding of $\jmb{x}_2$, and we wanted to keep the architecture for predicting $\jmb{S}^t$ in both the encoder/decoder symmetric. 

%this would be beyond what $\jmb{h}^t_1, \jmb{h}^t_2$ can provide since the primary purpose of $\jmb{h}^t_1, \jmb{h}^t_2$ is to reconstruct the stereo pair. Examples of $\jcb{\gamma}$ could include sparse lidar points if they are available, or the output of a decoded SGBM disparity map. In our case, we do not assume the existence of lidar points for every stereo pair, nor do we wish to utilize additional bits to store disparity estimates. Instead, 


\paragraph{Putting it all together}
The combined skip function, convolution, and activation layer $f^t$ in $D_2$ can be viewed as 
\begin{equation}
\begin{aligned} \label{eq:update}
\jmb{h}^{t+1}_2 = f^{t+1}(Conv(Concat(\jmb{h}^t_2, g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}))))
\end{aligned}
\end{equation}
%\slwang{$f$ is not defined.}
Here, we have presented skip functions in the decoder. 
% For our stereo compression models, w
We have similarly implemented skip functions in the encoder as well and found marginally better results. Our skip functions range from levels $l=1,2,3$, where $l=4$ represents the final reconstruction of the image $\hat{\jmb{x}}_1, \hat{\jmb{x}}_2$. Hence, the maximum height/width of $\jmb{h}^t_1$, $\jmb{h}^t_2$ used in $g_l$ is $H/2, W/2$. 

In terms of the actual operations to predict $\jcb{\gamma}$ and $\jmb{S}^t$, we use convolutional layers + GroupNorm\cite{wu_groupnorm} + ReLU's as the building blocks for predicting and upsampling $\jcb{\gamma}(\bar{\jmb{y}}_1, t)$, concatenating $\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}(\bar{\jmb{y}}_1, t)$, and predicting $\jmb{S}^t$. A general illustration is given in Fig. \ref{fig:stereo_complex_model} but more specific details are given in our supplementary material.
%The context $\gamma$ is flexible. In our setting, we design $\gamma$ as  $\gamma(\bar{y_1}, l)$, a function of the first image code and the level. The output of $\gamma$ is an initial ``disparity volume" $S^{dinit}$ of dimensions $B \times C^{dinit} \times D \times H/16 \times W/16$. Our architecture consists of 3 levels of skip functions, and we ensure $C^{dinit}$ is divisble by 3: $S^{dinit}_{0:\frac{C^{dinit}}{3}}$ corresponds to $\gamma(\bar{y_1}, l=1)$, $S^{dinit}_{\frac{C^{dinit}}{3}:\frac{2C^{dinit}}{3}}$ corresponds to $\gamma(\bar{y_1}, l=2)$, etc. The intuition here is that different channel groups in $S^{dinit}$ correspond to different initial estimates of disparities at a given level. \slwang{rewrite this paragraph since it could be improved by a lot. Starts with intuition why you need a context and what could be encoded into a good context. Then what's the context module's arhictecture design. Some of the details could go to supp. Notations could be more clear.}
%\jerry{Did an initial pass of adding intuition, not sure what could go into supp}
We refer to our stereo model as the "Disparity Stereo Model", or DSM. 


\subsection{Conditional Entropy Model} \label{sec:entropy_model}
 
Although our skip functions help to encourage that the information present in the latent code of the residual is not present in the latent code of the base image, there exists a correlation between the latent code of the base image with the latent code of the residual. This is because 1) the skip functions are not perfect, and do not remove all redundant information, and \raquel{what does perfect mean in this setting?} 2) even the new information present in the residual image is not independent of the base image \raquel{talk about why}. As an example, in the context of autonomous vehicles a person present in the residual image but not the base is most likely standing on the street or a sidewalk; they are probably not floating above a car or the horizon. \raquel{mmm thats a weird example in this context. Is this really what you mean? or is it the displacement that makes the residual have more info that is required?}

In order to exploit these relationships, we develop a joint entropy model $p(\bar{\jmb{y}}_1,\bar{\jmb{y}}_2 ; \jcb{\phi})$ which takes into account the dependence of $\bar{\jmb{y}}_2$ on $\bar{\jmb{y}}_1$. \raquel{shouldnt we talking about H for entropy model?}
Inspired by \cite{minnen_jointpriors,balle_varhyperprior,theis_imgcomp_ae}, we maintain a fully factorized, independent entropy model for the base image code, but we model the residual code as conditionally independent given the base image code, with each element of the residual code modeled as a Gaussian mixture model (GMM) convolved with a uniform density: \raquel{add motivation for this choice}
% \begin{equation}
\begin{equation} \label{eq:stereo_entropy}
p(\bar{\jmb{y}}_1,\bar{\jmb{y}}_2 ; \jcb{\phi}) = p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\phi}_2) p(\bar{\jmb{y}}_1 ; \jcb{\phi}_1)
\end{equation}
where $p(\bar{\jmb{y}}_1 ; \jcb{\phi}_1)$ denotes the entropy model of the base image code and $p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\phi}_2)$ denotes the entropy model of the residual image code, which is condition on the base image. $\jcb{\phi}_1, \jcb{\phi}_2$ are the full set of parameters for each univariate distribution. \raquel{odd choice of notation, as $\phi$ is typically use for functions. Maybe use $\theta$, or something less confusing}
% \end{equation}
% \begin{equation}
Both entropy models are factorized into the product of each individual code's distribution. 
\raquel{this is an approximation, say why it makes sense}
For the base image code $\bar{\jmb{y}}_1$,
\begin{equation} \label{eq:ind_entropy}
p(\bar{\jmb{y}}_1 ; \jcb{\phi}_1) = \prod_i {p_{1, i}(\bar{y}_{1,i} ;  \jcb{\phi}_1)}
\end{equation}
where 
%\[p_{1, i}(y; \jcb{\phi}_1) = \left(q_{1, i} * \mathcal{U}(-\frac{1}{2}, \frac{1}{2}) \right)(y) = \int_{y - 0.5}^{y+0.5} q_{1, i}(y ; \jcb{\phi}_1) dy\] and $q_{1, i}(y ;  \jcb{\phi}_1)$ is a deep neural network outputting the probability density of a given code, 
\begin{equation} \label{eq:ind_entropy2}
\begin{aligned}
p_{1, i}(\bar{y}_{1,i}; \jcb{\phi}_1) = \left(q_{1, i} * \mathcal{U}(-\frac{1}{2}, \frac{1}{2}) \right)(\bar{y}_{1,i}) = \\ c_{1, i}(\bar{y}_{1,i} + \frac{1}{2}; \jcb{\phi}_1) - c_{1, i}(\bar{y}_{1,i} - \frac{1}{2}; \jcb{\phi}_1)
\end{aligned}
\end{equation}
\raquel{is this equation correct? weird parenthesis, no dependency on  $\phi$, you havent defined $ \mathcal{U}$, etc}
Here, $c_{1, i}(y ;  \jcb{\phi}_1)$ represents the cumulative density of some underlying density model $q_{1, i}$ of a given code; we directly parameterize $c_{1, i}(y ;  \jcb{\phi}_1)$ with a neural network. \raquel{explain what this choice means and why is a good idea}\raquel{use better notation, $f$ for function and $w$ for weights of nnets}
%$\mathcal{U}(-0.5, 0.5) = 1 \text{ if } |x| < 0.5$ otherwise 0 \jerry{Isn't this redundant? It's a uniform distribution. }. 
This means each code's final distribution is equal to a neural network density estimation convolved by a uniform density function. This formulation has been proven to be more efficient in modeling the distribution of latents, especially since we inject additive uniform noise to quantizer during training. \raquel{why is it the case? the reviewer will not understand}
We refer the reader to supplmentary material in \cite{balle_varhyperprior} for more details. 
% where $p(\bar{y}_{1, i})$ 
Similarly we have the following conditional entropy model for $\bar{\jmb{y}}_2$:
\begin{equation} \label{eq:cond_entropy}
p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\phi}_2 ) = \prod_i {p_{2, i}(\bar{y}_{2,i} | \bar{\jmb{y}}_1; \jcb{\phi}_2) % * \mathcal{U}(-\frac{1}{2},\frac{1}{2})
}
\end{equation}
where \[p_{2, i}(y) = \left(q_{2, i} * \mathcal{U}(-\frac{1}{2}, \frac{1}{2}) \right)(y)\]
Unlike the base image's entropy model, we model each individual pixel's density function $q_{2, i}$ as a Gaussian mixture:
\[
q_{2, i} = \sum_k{w_{ik} \mathcal{N}(\mu_{ik},\sigma^2_{ik})})
\]
\raquel{didnt we say this before already about GMM? the section is a bit redundant. }
where $w_{ik}$ represents our normalized weight per Gaussian in the mixture. $w_{ik}, \mu_{ik}, \sigma^2_{ik}$ are the output of a deep learnable function, which takes $\bar{y_1}$ as input and $\phi_{2i}$ as its parameters. In our experiments below, we set $k=6$, indicating the number of distributions in the mixture; we found that a mixture model increased performance slightly compared to a single Gaussian. 
%\slwang{todo: one sentence to explain the intuition}
%where $\bar{y}_{1, i}, \bar{y}_{2, i}$ are the $i$th code of the left image and right image, respectively. Following \cite{balle} we convolbe the non-parameteric density with a uniform distributed model to better match the marginal. 
%In practice ,we use GMM to represent each invidual univariate distribution. 
%\begin{equation}
%p(\bar{y}_{1,i} |  \jcb{\phi}_1)
%\end{equation}
%\begin{equation} \label{eq:cond_entropy}
%p(\bar{\jmb{y} }_2| \jcb{\phi}_2, \bar{\jmb{y}}_1) = \prod_i {((\sum_k{w_{ik} \mathcal{N}(\mu_{ik},\sigma^2_{ik})}) * \mathcal{U}(-\frac{1}{2},\frac{1}{2}))(\bar{y}_{2i})}
%\end{equation}

% \end{equation} 
% \begin{equation}

% \end{equation}
% \slwang{you don't have each mixture's weight? each mixture is equally weighted? just a $(y)$ in the end is not okay. It's better to explicitly show which part is a function of $\phi$ and $y$. E.g. $\mu(\phi, y)$; follow common practice to use $\mu$ for mean.} 
% \jerry{Added the mixture weight but I think there is a misunderstanding here. The (N * U) part means a normal convolved with a uniform density (not a multiplication), and the (y) means the probability value at (y) given this convolved distribution. It's the same notation that Balle uses, but I can try to make this more clear.} \slwang{it doesn't make a lot of sense here. Is it derived from bayes rule? If yes, try to make the derivation and assumption over parameterized probability more explict, otherwise it's difficult to follow. $i, k$ is not clear as well. }
% Each $y_i$ represents a single element of $\bar{\jmb{y}}$. 
% In our conditional GMM, $w_{ik}$ represents our normalized weight per Gaussian in the mixture. $w_{ik}, \mu_{ik}, \sigma^2_{ik}$ are a function of $\phi_{2i}, \bar{y_1}$. In our experiments below, we set $k=6$, indicating the number of distributions in the mixture. Finally, the $(*)$ oeprator represents a convolution, and we convolve each distribution with a standard uniform to better match the posterior code distribution, as in \cite{balle_varhyperprior}. More details about our entropy model architecture and structure of $p_{\bar{y}_{1i} | \phi_{1i}}$ are given in supplementary material. 

\subsection{Learning}
\raquel{make a subsection about learning, and add all details here. Revise text to reflect this}

The entropy model is trained to minimize the cross-entropy between its modeled distribution and the distribution of the encoded latents; this loss term is counted as part of the overall entropy term in our rate-distortion tradeoff loss function. Specifically,

\begin{equation}
\begin{aligned} \label{eq:total_loss}
D + \beta R = \mathbb{E}_{\jmb{x}_1, \jmb{x}_2 \sim p_{\jmb{x}}}[ \underbrace{{||\jmb{x}_1 - \hat{\jmb{x}}_1||}^2_2}_{\text{Distortion (Img. 1)}} + \underbrace{{||\jmb{x}_2 - \hat{\jmb{x}}_2||}^2_2}_{\text{Distortion (Img. 2)}} ] + \\ 
\beta \mathbb{E}_{\jmb{x}_1, \jmb{x}_2 \sim p_{\jmb{x}}}[\underbrace{-\log_2 p_{\hat{\jmb{y}_1}}(\hat{\jmb{y}_1})}_{\text{Rate (Code 1)}}  \underbrace{- \log_2 p_{\hat{\jmb{y}_2} | \hat{\jmb{y}_1}}(\hat{\jmb{y}_2} | \hat{\jmb{y}_1})}_{\text{Rate (Code 2)}}]
\end{aligned}
\end{equation} 
We tune $\beta$, the weight on the entropy loss, on a sliding scale roughly from 0.5 to 0.001 for the lower bitrate to higher bitrate models respectively. 
In order to enforce a target bitrate for a given model, we modify the R term in our loss function to be: \begin{equation}
\begin{aligned} \label{eq:target_entropy}
R = \max(\mathbb{E}_{x \sim p_x}[-\log_2 p_{\hat{y}}(\hat{y})], H_t)
\end{aligned}
\end{equation} 
where  $H_t$ is our desired target entropy calculated from the target bitrate. 
%\slwang{move to this target entropy part as a loss function in tech section. }

We refrained from implementing an autoregressive entropy model such as PixelRNN/PixelCNN \cite{oord_pixelrnn} as in \cite{minnen_jointpriors, mentzer_condprobimg} due to concerns about speed during the encoding/decoding process. We also attempted to implement a hyperprior as in \cite{balle_varhyperprior}, but found that we couldn't tune our compression model to converge to the desired results. 

%Instead, we implement the factorized prior entropy model as a baseline, which assumes independence between each dimension of the latent code, and can be represented as 
%\begin{equation}
%\begin{aligned} \label{eq:ind_entropy}
%p_{\bar{y} | \phi}(\bar{y} | \phi) = \prod_i {(p_{y_i | \phi_i} * \mathcal{U}(-\frac{1}{2},\frac{1}{2}))(\bar{y_i})}
%\end{aligned}
%\end{equation} 
%where our modeled distribution $p_{y_i | \phi_i}$ is convolved with a uniform density. \slwang{baseline goes to ablation, showcasing how conditional entropy improves. }

If the optimal bitrate for encoding $\hat{\jmb{y}_2}$ independent of $\hat{\jmb{y}_1}$ is given by $H(\hat{\jmb{y}_2})$ (Shannon's source coding theorem), then the optimal bitrate for $\hat{\jmb{y}_2}$ conditioned on $\hat{\jmb{y}_1}$ is $H(\hat{\jmb{y}_2} | \hat{\jmb{y}_1})$. Then the maximum amount of information we can possibly "extract" from $\hat{\jmb{y}_1}$, or in other words, the maximum amount of bitrate savings we can achieve for $\hat{\jmb{y}_2}$, is upper bounded by $H(\hat{\jmb{y}_2}) - H(\hat{\jmb{y}_2} | \hat{\jmb{y}_1}) = I(\hat{\jmb{y}_1}, \hat{\jmb{y}_2})$, or the mutual information between $\hat{\jmb{y}_1}, \hat{\jmb{y}_2}$. 

In theory, if our residual entropy model $p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\phi}_2 )$ was expressive enough, we could reduce the cross-entropy with the "true" probability distribution $p^*(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1 )$ without the need for any skip functions in the previous sections. A similar thought could be applied to video compression, similar to \cite{han_vid_deepprob}, removing the need for motion compensation and residual compression. But it has been shown that more expressive entropy models oftentimes require complex autoregressive models \cite{minnen_jointpriors}, which again are inefficient during inference. In our experiments, we analyze the extent to which our skip functions and conditional entropy complement each other in terms of bitrate savings. While there is a certain degree of cannibalization, we still show in below experiments that combining skip functions with our conditional entropy model yields the best results for all bitrates.

%\slwang{Could we do any empirical exp to justify this?}


%\subsection {Trying traditional motion-compensated residuals as a baseline}
%As a separate baseline, we try porting traditional video-compression techniques into the stereo setting. We set $x_1$ as our reference frame, so $x_1$ is compressed using the Balle single-image compression baseline. $x_2$ is compressed similar to a P-frame. We first use SGBM to generate motion estimates $m$ to warp $\hat{x}_1$ (the reconstructed first image) to the camera frame of $x_2$. Then, we compress $m$ using a second Balle single-image network, getting $\hat{m}$ as the reconstructed motion estimates. Finally, we compress $x_2 - \hat{x_1}^{\hat{m}}_1$ using a third Balle single-image network, where $\hat{x_1}^{\hat{m}}_1$ is the motion-warped $\hat{x}_1$ as $\hat{x}^m_1$, using the decompressed motion estimates. 


==> method.tex <==
% !TEX root = top.tex
% In section: Approach
\section{Deep Stereo Compression}

In this paper we tackle the problem of compressing a pair of stereo images. % that have overlapping fields of view. 
Intuitively, if the overlapping field of view  between the stereo  pair 
is very high, then the bitrate of the combined latent code should be lower than the sum of the bitrates if we compressed the images separately; at the very least it cannot be higher. More formally, let us denote $\jmb{x}_1, \jmb{x}_2$ as a pair of rectified stereo images and let $H(\jmb{x}_1, \jmb{x}_2)$ be the entropy of the stereo pair. Given the fact that the content of two images are highly correlated, the mutual information $I(\jmb{x}_1, \jmb{x}_2) = H(\jmb{x}_1) + H(\jmb{x}_2) - H(\jmb{x}_1, \jmb{x}_2) > 0$. 


This observation motivates our general approach: we propose a single compression model that jointly compresses two stereo images. Towards this goal, we focus on extracting as much information as possible from one image in order to reduce the bitrate in the second, such that the total bitrate is lower than the result of independent single-image compression. Our approach is a two-stream deep encoder-decoder network as shown in Fig.~\ref{fig:stereo_complex_model}. Two images are passed to an encoder and quantizer to get a discretized latent code; then, a decoder is utilized to reconstruct the image from the latent code. Compared to previous deep image compression networks, we have two major contributions: 1) we add \textit{multi-level, parametric skip functions} from the first image's feature maps to propagate useful feature content to the second image; 2) we utilize a conditional entropy model to better model the correlation between the latent code of the two images. Next we will describe the details of each component. 
 
 
 \subsection{Encoding/Decoding and Quantization} \label{sec:feature_map}
Our encoder, decoder, and quantizer functions % \raquel{its a trio, not pair ;)} 
borrow their architectures from the factorized prior single-image compression model in Ball\'e et al. \cite{balle_varhyperprior}.  As shown in Fig.~\ref{fig:stereo_complex_model}, each encoder is implemented with a series of 4 downsampling convolutions (by 2x) and  Generalized Divisive Normalization (GDN) layers \cite{balle_gdn}. Each decoder is implemented with a series of 4 upsampling deconvolutions (by 2x) and Inverse-GDN layers. Each quantizer $Q$ applies a rounding function to the floating-point output of the encoder $Q(E(\jmb{x})) = Q(\jmb{y}) = \hat{\jmb{y}}$ to output the binary code representation. 
The dimension of $\hat{\jmb{y}}$ is $M \times H/16 \times W/16$. 
% Similar to \cite{balle_imgcomp_end2end, balle_varhyperprior}, the quantizer applies additive uniform noise during training $Q(\jmb{y}) = \bar{\jmb{y}}$. \raquel{its odd that you are talking about training here, while you havent talk about loss function or anything. Ill pass this to learning subsection}
% However, similar to \cite{lee_contextadapt}, we use $\hat{\jmb{y}}$ as the input into the decoder and only use $\bar{\jmb{y}}$ as input into our entropy model (Section \ref{sec:entropy_model}); we found that this yielded a smaller discrepancy in error metrics between training and inference. 
% Please refer to the supplementary material for more detailed computation graph of each module. \raquel{this is hard to understand since you havent define anything yet...}
 
 
%% \raquel{say why this makes sense}
%, as well as learning a \textit{conditional entropy model}. Our skip functions help to improve reconstruction quality for a given bitrate by extracting information
%from the feature maps of the first image, while our conditional entropy model models the inherent dependence of the residual code with the reference code. 
%\raquel{rewrite the paragraph to explain one after another, instead of first saying both and then explaining. Its easier to read}
%The two components are based on the following facts respectively: 1) features from a stereo pair are more related if we warp one with a good disparity estimation; 2) the codes of two images are dependent given the dependence of the input. \raquel{this hould be pass at the begining of this paragraph where you give context avbout the two components not at the end.}

\subsection{Parametric Skip Function} \label{sec:vol_disparity}
To reduce the joint bitrate across the stereo pair, we design network modules called \textit{parametric skip functions} to propagate information from the first image's encoder/decoder to the second.
%connect the two images' encoder/decoder. This allows information to be propagated from one to the other. 
%We conjecture that for feature correlation between a stereo pair will happen across all the levels of feature maps. Moreover, through estimating the disparity between the stereo images, we could further warp features with disparity and improve the pixel-level alignment between features from two images, making the information passed towards the accurate local target.  Motivated by this, we propose a multi-level skip function to fuse information from both images at each level. 
We conjecture that for a given stereo pair, there exists a correlation between the feature maps of the two images at all levels in the encoder and decoder. Moreover, if we estimate the disparity between each pair of feature maps, we can warp one feature to the other and improve the pixel-level alignment between the two feature maps; this in turn allows us to pass information from one feature map accurately to the corresponding spatial positions of the other. 


% We have two types of skip connections across all levels. Let us denote $\jmb{h}^t_1, \jmb{h}^t_2$ as feature maps at a given level $t$ for the first and second image, respectively. The first type of skip connection is from a first image's feature level $\jmb{h}^t_1$ to the second image's next level $\jmb{h}^{t+1}_2$, as shown as {\color{red}\textbf{red}} arrows in Fig.~\ref{fig:stereo_complex_model}. This is refered to as feature-feature skip connection, passing the level-specific information. The second type links the quantized code $\hat{\jmb{y}}_1$ to all the features in the second image's encoder-decoder as shown as {\color{orange}\textbf{orange}} arrows in Fig.~\ref{fig:stereo_complex_model}. This passes global information about the left image to each layer.  
Specifically, in order to compute the feature map of the second image at level $t$, each skip function takes its previous layer's feature $\jmb{h}^{t-1}_2$, the previous layer feature from image one $\jmb{h}^{t-1}_1$ and the first image's code $\hat{\jmb{y}}_1$ as input. Each skip function module consists of four parts. First, a fully convolutional \textbf{global context} encoding module $f(\hat{\jmb{y}_1}; \jmb{w})$ encodes the first image's latent code to a feature descriptor $\jmb{d}_1$ capturing global context information of image 1, contained in its latent code. The global context feature is shared across all the different levels.  Secondly, a \textbf{stereo cost volume} module estimates a cost volume $\jmb{c}^{t-1}$ from the input of the first feature map, right feature map \raquel{you mean second feature map?} and the encoded context. 
The cost volume's size is $D\times H^{t-1} \times W^{t-1}$ where $D$ is the maximum disparity and $H^{t-1}$ and $W^{t-1}$ are the height/width of $\jmb{h}^{t-1}_1$. 
A softmax layer is applied to ensure the cost is normalized along the disparity dimension per pixel. Each value in the cost volume can be seen as a probability/confidence measure of the correct disparity at that coordinate. We then use this cost volume to \textbf{densely warp} the feature from image 1 to image 2. Particularly, per each pixel $i$ the new feature vector is computed through a weighted sum of feature vectors across all  disparity values:
\[
\jmb{g}^{t-1}_{2, i} = \sum_d c_{d, i} \cdot \jmb{h}^{t-1}_{1,(i,d)}
\]
where $c_{d, i}$ represents the cost of disparity $d$ at pixel $i$. $(i,d)$ represents the pixel index that is $d$ pixels right of pixel $i$. The volumetric warping gives us a warped feature map $\jmb{g}^{t-1}_{2}$ which better aligns with image 2. This design is conceptually similar to previous appearance synthesis papers such as \cite{flynn_deepstereo, xie_deep3d}. Compared to regressing a single disparity map and warping with bilinear sampling \cite{jaderberg_spatialtransform}, our design allows more flexible connections between the target pixel and a disparity range of pixels from the source image.  Finally, we use an \textbf{aggregation} function to predict the feature map as the final output of our parametric skip function:
\[
\jmb{h}^{t}_2 = a(\jmb{g}^{t-1}_{2}, \jmb{h}^{t-1}_2)
\] with $\jmb{g}^{t-1}_{2, i}$  the volumetric warped feature from image 1 and $\jmb{h}^{t-1}_2$ the previous layer's feature from image 2. For the architecture details of context encoding, stereo cost volume and aggregation, please refer to our supplementary material.  \slwang{todo: we need to update the figure of this part accordingly to reflect the four parts. } 

\subsection{Conditional Entropy Model} \label{sec:entropy_model}
\begin{figure}
	\centering
	\includegraphics[width=.9\linewidth]{figures/disp_vis.pdf}
	\caption{Visualization of the disparity volumes at each resolution level in the encoder/decoder, by taking the mode over the disparity dimension for each feature pixel. Tiling effects are inherently due to unsupervised training on crops.}
	\label{fig:disp_vis}
	\vspace{-2mm}
\end{figure}
% \jerry{I'm wondering if we should bring up the fact that we didn't implement a hyperprior / autoregressive model here. Raquel, any thoughts?} 
% \jerry{Also Shenlong asks why we didn't try these other approaches: 1) modeling the first image with a Gaussian, or 2) if we use the factorized prior for the first image, why we didn't also directly model the CDF with a neural net for the conditional entropy. As background: the Ball\'e model used a factorized prior that directly modeled the CDF, and showed that it was better than the Theis model which used a fixed Gaussian. The hyperprior model in Ball\'e instead used a Gaussian, which is what my conditional entropy is based on.}

%Modeling the entropy of the quantized code accurately is critical to navigate the rate-distortion trade-off, as entropy the theoretical guidance of bitrate \cite{entropy-coding}. 
Accurately modeling the entropy of the quantized code is critical in navigating the rate-distortion trade-off, as entropy is a tight lower bound of bitrate \cite{shannon_lowerbound}. 
%As discussed in Sec.~\ref{sec:overview}, 
There exists a correlation between the latent codes of the two images, given the highly correlated image content. In order to exploit these relationships, we develop a joint entropy model with neural networks to estimate the joint distribution of the code. In order to maintain differentiability while mimicking the effect of rounding errror during quantization, we consider a noisy version of $\jmb{y}$ as input: $\bar{\jmb{y}} = \jmb{y} + \jmb{z}$, where $\jmb{z} \sim \mathcal{U}(-0.5, 0.5)$. Thus our goal is to model the joint distribution $p(\bar{\jmb{y}}_1,\bar{\jmb{y}}_2 ; \jcb{\theta})$ which takes into account the dependence of $\bar{\jmb{y}}_2$ on $\bar{\jmb{y}}_1$. Specifically, we factorize the joint probability into the prior probability over $\bar{\jmb{y}}_1$ and conditional probability of $\bar{\jmb{y} }_2$ given  $\bar{\jmb{y}}_1$:
\begin{equation} \label{eq:stereo_entropy}
p(\bar{\jmb{y}}_1,\bar{\jmb{y}}_2 ; \jcb{\theta}) = p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\theta}_2) p(\bar{\jmb{y}}_1 ; \jcb{\theta}_1)
\end{equation}
where $p(\bar{\jmb{y}}_1 ; \jcb{\theta}_1)$ denotes the probability 
%probability density function (PDF) 
of the first image code and $p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\theta}_2)$ denotes the probability
%PDF 
of the second image code, which is conditioned on the first image. $\jcb{\theta}_1, \jcb{\theta}_2$ are the full set of parameters for each univariate distribution. 
% \raquel{odd choice of notation, as $\theta$ is typically use for functions. Maybe use $\theta$, or something less confusing}
 Inspired by \cite{minnen_jointpriors,balle_varhyperprior,theis_imgcomp_ae}, to make computation feasible, both models are factorized into the product of each individual code's distribution under the full independence and conditional independence assumptions: 
% \raquel{this is an approximation, say why it makes sense}
% For the base image code $\bar{\jmb{y}}_1$,
Specifically,
\begin{align} \label{eq:ind_entropy}
p(\bar{\jmb{y}}_1 ; \jcb{\theta}_1) &= \prod_i {p_{1, i}(\bar{y}_{1,i}; \jcb{\theta}_1)}\\
 p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\theta}_2 ) &= \prod_i {p_{2, i}(\bar{y}_{2,i} | \bar{\jmb{y}}_1; \jcb{\theta}_2)} % * \mathcal{U}(-\frac{1}{2},\frac{1}{2})
\end{align}
%However, a deep parametric function might not be suitable for modeling PDFs with a discontinuity shape, e.g. a uniform distribution between [-0.5, 0.5]. This restricts the power of the entropy model. Following previous work \cite{balle_varhyperprior}, we overcome this issue by designing the parametric PDF $p_{1, i}(y; \jcb{\theta}_1)$ as follows:
However, directly modeling a probability density function (PDF) with a deep parametric function may not be suitable for PDFs with discontinuous shapes, e.g. a uniform distribution between [-0.5, 0.5]. This restricts the power of the entropy model. Following previous work \cite{balle_varhyperprior}, we overcome this issue by designing our probability model $p_{1, i}(y; \jcb{\theta}_1)$ as follows:
\begin{equation} \label{eq:ind_entropy2}
\begin{aligned}
p_{1, i}(y; \jcb{\theta}_1) & = \left(q_{1, i} * u \right)(y) 
\end{aligned}
\end{equation}
where $u(\tau) = 1 $ if $|\tau| < 0.5$ otherwise $u(\tau) = 0$. $*$ is the convolution between two functions. Thus we have:
\begin{equation} \label{eq:ind_entropy2}
\begin{aligned}
p_{1, i}(y; \jcb{\theta}_1) &  =\int_{-\infty}^{\infty} q_{1, i}(\tau; \jcb{\theta}_1) u(y - \tau) d\tau
\\&  =\int_{y-0.5}^{y+0.5} q_{1, i}(\tau; \jcb{\theta}_1) d\tau \\
 & = c_{1, i}(y+ 0.5; \jcb{\theta}_1) - c_{1, i}(y - 0.5; \jcb{\theta}_1)
\end{aligned}
\end{equation}
where $c_{1, i}(y; \jcb{\theta}_1)$ is the cumulative density function (CDF) of some underlying PDF $q$.
%In practice, we just need to use a neural network to model $c_{1, i}(y; \jcb{\theta}_1)$ in order to get the final PDF $p_{1, i}(y; \jcb{\theta}_1)$.  
This intuitively means that we can define $p_{1, i}(y; \jcb{\theta}_1)$ as an area under the CDF rather than directly as the PDF, and we can use a neural network to directly model $c_{1, i}(y; \jcb{\theta}_1)$. This approach has better capacity to model steep edge PDFs, since even for steep edged PDF, the CDF is still continuous. 
Similarly, we have the conditional probability for each code of image 2: 
\begin{equation}
p_{2, i}(y|\bar{\jmb{y}}_1; \jcb{\theta}_1)  = \left(q_{2, i} * u \right)(y) 
\end{equation}
 Unlike the base image's entropy model, we model each individual pixel PDF $q_{2, i}$ as a Gaussian mixture:
\[
q_{2, i} = \sum_k{w_{ik} \mathcal{N}(\mu_{ik},\sigma^2_{ik})})
\]
where $w_{ik}, \mu_{ik}, \sigma^2_{ik}$ are the distribution parameters depending on $\bar{\jmb{y}}_1$ and $ \jcb{\theta}_2$. We also rewrite the convolution as the difference between CDF as in Eq.~\ref{eq:ind_entropy2}. The CDF of a GMM is generally computed numerically in most computational frameworks, while the derivative is analytical. Thus we just need to learn a function that predicts parameters  $w_{ik}, \mu_{ik}, \sigma^2_{ik}$ given $\bar{\jmb{y}}_1$ with $\jcb{\theta}_2$ as learnable parameters, instead of modeling the CDF value directly as in the base image's entropy model. We found that a mixture model increased performance slightly thanks to its stronger capability. 

\begin{figure*}
	\centering
	\includegraphics[height=0.3\linewidth]{figures/tor4d_msssim.pdf}
        \includegraphics[height=0.3\linewidth]{figures/tor4d_psnr.pdf}
	\includegraphics[height=0.3\linewidth]{figures/tor4d_msssim_db.pdf} \\
	\includegraphics[height=0.3\linewidth]{figures/city_msssim.pdf}
        \includegraphics[height=0.3\linewidth]{figures/city_psnr.pdf}
	\includegraphics[height=0.3\linewidth]{figures/city_msssim_db.pdf}
	\caption{Plot of DispSkip with conditional entropy against single-image compression baselines, for TOR4d and Cityscapes.}
	\vspace{-4mm}
	\label{fig:main_results_figure}
\end{figure*}

\subsection{Learning}
% \raquel{make a subsection about learning, and add all details here. Revise text to reflect this}
Our model is trained end-to-end to minimize the following objective function: 
\begin{equation}
\begin{aligned} \label{eq:total_loss}
\ell + \beta R = \mathbb{E}_{\jmb{x}_1, \jmb{x}_2 \sim p_{\jmb{x}}}[ \underbrace{{||\jmb{x}_1 - \hat{\jmb{x}}_1||}^2_2}_{\text{Distortion (Img. 1)}} + \underbrace{{||\jmb{x}_2 - \hat{\jmb{x}}_2||}^2_2}_{\text{Distortion (Img. 2)}} ] + \\ 
\beta \mathbb{E}_{\jmb{x}_1, \jmb{x}_2 \sim p_{\jmb{x}}}[\underbrace{-\log_2 p(\bar{\jmb{y}}_1; \jcb{\theta})}_{\text{Rate (Code 1)}}  \underbrace{- \log_2 p(\bar{\jmb{y}}_2 | \bar{\jmb{y}}_1; \jcb{\theta})}_{\text{Rate (Code 2)}}]
\end{aligned}
\end{equation} 
where the first term encodes reconstruction quality of both images and the second term is the bitrate term with the rate predicted by the entropy model. 
%Since $\hat{\jmb{y}}_1 = Q(E(\jmb{x}))$, where $Q(\cdot)$ is the non-differentiable function. It is non-trivial to do back-propagate through $\jmb{y}$ directly. Instead, we use the a `noisy' yet differentiable real-valued approximation as during learning instead of the quantized code: $\bar{\jmb{y}} = E(\jmb{x}) + \jmb{z}$, where $\jmb{z} \sim \mathcal{U}(-0.5, 0.5)$. 
We tune the balancing parameter $\beta$, the weight on the entropy loss, on a sliding scale roughly from 0.5 to 0.001 to get the lower bitrate to higher bitrate models respectively. 

% The entropy model is trained to minimize the cross-entropy between its modeled distribution and the distribution of the encoded latents; this loss term is counted as part of the overall entropy term in our rate-distortion tradeoff loss function. Specifically,
As an alternative, we could enforce a target bitrate for a given model by modifying the rate function to be: \begin{equation}
\begin{aligned} \label{eq:target_entropy}
%R = \max(\mathbb{E}_{x \sim p_x}[-\log_2 p_{\hat{y}}(\hat{y})], H_t)
R = \max(\mathbb{E}_{\jmb{x}_1, \jmb{x}_2 \sim p_{\jmb{x}}}[-\log_2 p(\bar{\jmb{y}}_1, \bar{\jmb{y}}_2; \jcb{\theta})], H_t)
\end{aligned}
\end{equation} 
where  $H_t$ is our desired target entropy calculated from the target bitrate. 
%\slwang{move to this target entropy part as a loss function in tech section. }

% We refrained from implementing an autoregressive entropy model such as PixelRNN/PixelCNN \cite{oord_pixelrnn} as in \cite{minnen_jointpriors, mentzer_condprobimg} due to concerns about speed during the encoding/decoding process. We also attempted to implement a hyperprior as in \cite{balle_varhyperprior}, but found that we couldn't tune our compression model to converge to the desired results. 

%Instead, we implement the factorized prior entropy model as a baseline, which assumes independence between each dimension of the latent code, and can be represented as 
%\begin{equation}
%\begin{aligned} \label{eq:ind_entropy}
%p_{\bar{y} | \theta}(\bar{y} | \theta) = \prod_i {(p_{y_i | \theta_i} * \mathcal{U}(-\frac{1}{2},\frac{1}{2}))(\bar{y_i})}
%\end{aligned}
%\end{equation} 
%where our modeled distribution $p_{y_i | \theta_i}$ is convolved with a uniform density. \slwang{baseline goes to ablation, showcasing how conditional entropy improves. }

% If the optimal bitrate for encoding $\hat{\jmb{y}}_2$ independent of $\hat{\jmb{y}}_1$ is given by $H(\hat{\jmb{y}}_2)$ (Shannon's source coding theorem), then the optimal bitrate for $\hat{\jmb{y}}_2$ conditioned on $\hat{\jmb{y}}_1$ is $H(\hat{\jmb{y}}_2 | \hat{\jmb{y}}_1)$. Then the maximum amount of information we can possibly "extract" from $\hat{\jmb{y}}_1$, or in other words, the maximum amount of bitrate savings we can achieve for $\hat{\jmb{y}}_2$, is upper bounded by $H(\hat{\jmb{y}}_2) - H(\hat{\jmb{y}}_2 | \hat{\jmb{y}}_1) = I(\hat{\jmb{y}}_1, \hat{\jmb{y}}_2)$, or the mutual information between $\hat{\jmb{y}}_1, \hat{\jmb{y}}_2$. 

% In theory, if our residual entropy model $p(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1; \jcb{\theta}_2 )$ was expressive enough, we could reduce the cross-entropy with the "true" probability distribution $p^*(\bar{\jmb{y} }_2| \bar{\jmb{y}}_1 )$ without the need for any skip functions in the previous sections. A similar thought could be applied to video compression, similar to \cite{han_vid_deepprob}, removing the need for motion compensation and residual compression. But it has been shown that more expressive entropy models oftentimes require complex autoregressive models \cite{minnen_jointpriors}, which again are inefficient during inference. In our experiments, we analyze the extent to which our skip functions and conditional entropy complement each other in terms of bitrate savings. While there is a certain degree of cannibalization, we still show in below experiments that combining skip functions with our conditional entropy model yields the best results for all bitrates.


%% \raquel{we need a paragraph stating what we are going to see in this section and the intuitions. Its hard to follow for someone that doesnt know what you have done}
%
%\paragraph{General Skip Function Structure:}, where $\jmb{h}^t_1, \jmb{h}^t_2$ are the feature maps in $D_1$ and $D_2$ at a given level $t$, and $\jcb{\gamma}$ is a function of the main image code and incorporates global context information. \raquel{yes we can do that but you need to say why this is a good idea. Give always motivation of your choices to help the reviewer understand why what you did makes sense}
%Details for $\jcb{\gamma}$ described at the end of Sec. \ref{sec:vol_disparity}. \raquel{this is odd as this is that section!}
%%\slwang{define $\gamma$ more formally / specifically}
%Each skip function output is  concatenated with the feature map at $D_2$ before the next upsampling convolution. 
%% We denote $g_l$ as a skip function rather than a skip connection because while $g_l$ could be modeled as a traditional skip connection (an identity function $(g_l(h^t_1, h^t_2, \gamma) = h^t_1$, it can be any arbitrary function. 
%Note that the skip function is a generalized case of skip connection in residual modules. 
%It is degraded to standard skip connections when $g_l$ is an identity function ($g_l(\jmb{h}^t_1, 
%\jmb{h}^t_2, \jcb{\gamma}) = \jmb{h}^t_1$). In our experiments, we show that a nonlinear deep warping function increases the flexibility of how information is propagated from one image to the other. \raquel{maybe say form reference image to X image. As current sentence sort of hints symmetry, which is not}
%\raquel{we need a fancy name for this skip functions. Parametric skip functions? Or something}
%% We denote $g_l$ as a skip function rather than a skip connection because while $g_l$ could be modeled as a traditional skip connection (an identity function $(g_l(h^t_1, h^t_2, \gamma) = h^t_1$, it can be any arbitrary function. 
%
%%Hence the combined skip function, convolution, and activation layer $f_l$ in $D_2$ can be viewed as 
%%\begin{equation}
%%\begin{aligned} \label{eq:update}
%%\jmb{h^{l+1}_2} = f_{l+1}(Conv(Concat(\jmb{h}^t_2, g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}))))
%%\end{aligned}
%%\end{equation}
%%%\slwang{$f$ is not defined.}
%%Here, we have presented skip functions in the decoder. 
%%% For our stereo compression models, w
%%We have similarly implemented skip functions in the encoder as well and found marginally better results. Our skip functions range from levels $l=1,2,3$, where $l=4$ represents the final reconstruction of the image $\hat{\jmb{x}}_1, \hat{\jmb{x}}_2$. Hence, the maximum height/width of $\jmb{h}^t_1$, $\jmb{h}^t_2$ used in $g_l$ is $H/2, W/2$. 
%
%%In the simplest case, we do model $g_l$ as an identity function, so effectively each $h^t_1, h^t_2$ is concatenated into a convolutional layer in $D_2$. This can work to a degree if the baseline between the stereo pair is not too wide and there exists shared information within a few pixels of each other between the two images. We refer to this model as the ``Simplified Stereo Model" (SSM). \slwang{Given complext model has better performance, probably we should move the this paragraph ssm to ablation study instead, showcasing skip function is better than skip connection in our model, instead of proposing two models.}
%%\jerry{Removed the SSM paragraph, will put into experiments/ablation.}
%
%%\subsection{Volumetric Disparity-warped skip functions} \label{sec:vol_disparity}
%
%\paragraph{Predicting Volumetric Disparities for Feature Warping:}
%In our skip functions, we aim to obtain good disparity estimates between a stereo pair to better warp feature maps between $E_1,D_1$ to $E_2,D_2$. But there are a few caveats and considerations. First, we  designed our skip functions to be present at every feature map resolution. This is due to the fact that  feature maps at each level in $E,D$ contain different layers of high-level and low-level information. Thus  the optimal disparity estimates to warp a feature map at one level in $E_1,D_1$ for $E_2,D_2$ may not be the optimal estimates at another level.
%
%Moreover, as mentioned in Section \ref{sec:related_work}, existing stereo matching networks are inefficient and suboptimal, especially with the absence of ground-truth depth to train the network. \raquel{why are we talking about absence of GT?}
%We found that using a separate stereo matching network to predict disparities at each level quickly overstepped GPU memory limits, and that using a single stereo matching network to predict disparities for all resolution levels produced suboptimal results. 
%
%%\slwang{the above two subsections are not well structured. we might want to make some changes, perhaps merge here. } \jerry{Tried to do some rearranging.}
%
%
%%\begin{figure*}
%%	\centering
%%	\includegraphics[width=\linewidth]{figures/bilinear_ex.png}
%%	\caption{Demonstration of a failure case for bilinear sampling when training disparities on a consistency/photometric loss. Given the green point in camera 2, the plots demonstrate the photometric loss given a disparity (in the leftward x-direction) from the same point in camera 1. The correct disparity (as well as the minimum) is given by the green line, and the predicted disparity is given by the blue dot. The disparity update vector is shown by the blue arrows. In (b), bilinear sampling only provides information on the neighboring pixel values, and so the disparity is pushed further to the right. In (c), the disparity volume (purple region) contains information of all pixels within its range (starting from 0), which contains the ideal minimum, and the gradient pushes the disparity closer to the true value.}
%%	\label{fig:bilinear_ex}
%%\end{figure*}
%
%In order to use disparities to extract the right feature information at each level, we propose skip functions that predicts and makes use of \textit{volumetric} disparity estimates. Each skip function first outputs a cost volume $\jmb{S}^t = s_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma})$ of dimension $B \times D \times H^t \times W^t$, where $B$ is batch size and $D$ is the disparity range. Each value in the cost volume can be seen as a probability/confidence measure of the correct disparity at that coordinate. Then, if $C^t$ is the channel dimension of $\jmb{h}^t_1$, we also expand $\jmb{h}^t_1$ into a volumetric representation $\jmb{V}^t_1$ of size $B \times C^t \times D \times H^t \times W^t$, where each disparity dimension represents $\jmb{h}^t_1$ offset by disparity $d$. The cost volume is then used to ``select" values from $\jmb{V}^t_1$. This skip function can be represented as the following: 
%
%%\slwang{define B, C, H, W, V otherwise} \jerry{V is defined; H/W are pretty obvious; I'll define B/C}.
%
%\begin{equation}
%\begin{aligned} \label{eq:complex_skip}
%g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}) = \sum_{d=0}^{D}{\jmb{S}^t_d \cdot
%	\jmb{V}^t_{1d}} 
%\end{aligned}
%\end{equation}
%%\slwang{talk about if you ensure the cost is non-negative and if cost is normalized in any form. You haven't talk about $S^t$'s architecture as well} \jerry{Architecture is briefly described in the last paragraph of this section but not sure if it can be moved to supp.}
%We apply a softmax across every disparity dimension in $\jmb{S}^t$, so each value represents a probability estimate of disparity $d$ in pixel position $0 \leq i,j \leq W^t, H^t$. 
%Our approach of directly using the cost volumes for sampling is similar to those of appearance synthesis papers, such as \cite{xie_deep3d,flynn_deepstereo}, but to our knowledge this is the first time this has been used for compression. Since we regress a separate cost volume at each level $t$, we allow for more flexible spatial relationships amongst the different feature map levels. 
%
%%Finally, we have observed both theoretically and empirically that bilinear sampling, a tool used in stereo matching and depth estimation to sample images in another frame using disparity estimates, is not suitable for learning disparities. Every since \cite{jaderberg_spatialtransform} showed that bilinear sampling was a locally differentiable operation, different papers \cite{godard_leftright, garg_depthest, zhong_selfsupstereo} have used bilinear sampling to learn disparities using photometric loss and left-right consistency loss. However, we observe that bilinear sampling and related sampling kernels by definition do not obtain information beyond the immediately adjacent pixels to the disparity estimates. As a result, it is incredibly difficult for the proper disparity to be learned if the proper disparity falls more than a few pixels beyond the current disparity estimate.
%%See Fig. \ref{fig:bilinear_ex} for an illustration of this problem. 
%%\slwang{I am a bit worried about this claim since there are quite a few unsupervised learning approach using photometric loss over bilinear sampled warping as supervision. People can easily question here since we don't given enough convincing evidence. I am leaning towards to rephrasing this as that disparity volume warping build connections from more pixels from left image to a target pixel at right than bilinear interpolation. So from architecture perspective not optimization perspectives} 
%%\jerry{Commented out the relevant chunk of text - I tried to rewrite this a little bit.}
%
%We also considered directly regressing the disparity estimate from the cost volume, and then using bilinear sampling as in \cite{jaderberg_spatialtransform} to warp the feature maps in a differentiable manner, similar to \cite{zhong_selfsupstereo, godard_leftright, garg_depthest}. However we found that directly using the cost volume for feature selection allowed the model to learn a more flexible weighted arrangement between an entire disparity range of pixels instead of just between two. Also, we empirically observed that since bilinear sampling kernels are only locally differentiable between two adjacent pixels, we found it hard to tune our compression models to learn any meaningful disparities in this manner, even when trained with additional regularization such as smoothness. (TODO: put in supp?) 
%%Using a cost volume for sampling instead of regressing a disparity estimate first bypasses the local differentiability problem presented by bilinear sampling kernels. 
%\paragraph{Incoporating Global Context for Disparity Prediction}
%We've defined $\jmb{S}^t$ as a function of $\jmb{h}^t_1, \jmb{h}^t_2$ and a context term $\jcb{\gamma}$. The goal of $\jcb{\gamma}$ is to incorporate global or external information to better learn $\jmb{S}^t$; we've designed $\jcb{\gamma}$ as $\gamma(\bar{\jmb{y}}_1, l)$, a function of the first image code and the current level.  The output of $\jcb{\gamma}(\bar{\jmb{y}}_1, l)$ is an ``initial disparity volume" $\jmb{S^{\gamma_l}}$ of dimensions $B \times C^{\jcb{\gamma_l}} \times D \times H/16 \times W/16$. By taking in $\bar{\jmb{y}}_1$ as input, $\gamma(\bar{\jmb{y}}_1, l)$ offers our network a view of the global image context - moreover, $\gamma$ provides separate pathways to learn an initial ``monocular" estimate of the disparities at each level, based on $\bar{\jmb{y}}_1$, before being concatenated with $\jmb{h}^t_1, \jmb{h}^t_2$ to predict the final $\jmb{S}^t$. The pathways to predict $\jcb{\gamma}$ from $\bar{\jmb{y}}_1$ and $t$ are solely focused on learning disparities and not reconstruction, unlike those forming $\jmb{h}^t_1, \jmb{h}^t_2$. We could not include $\bar{\jmb{y}}_2$ as an input into $\jcb{\gamma}$ because $\jmb{S}^t$ is used during the encoding of $\jmb{x}_2$, and we wanted to keep the architecture for predicting $\jmb{S}^t$ in both the encoder/decoder symmetric. 
%
%%this would be beyond what $\jmb{h}^t_1, \jmb{h}^t_2$ can provide since the primary purpose of $\jmb{h}^t_1, \jmb{h}^t_2$ is to reconstruct the stereo pair. Examples of $\jcb{\gamma}$ could include sparse lidar points if they are available, or the output of a decoded SGBM disparity map. In our case, we do not assume the existence of lidar points for every stereo pair, nor do we wish to utilize additional bits to store disparity estimates. Instead, 
%
%
%\paragraph{Putting it all together}
%The combined skip function, convolution, and activation layer $f^t$ in $D_2$ can be viewed as 
%\begin{equation}
%\begin{aligned} \label{eq:update}
%\jmb{h}^{t+1}_2 = f^{t+1}(Conv(Concat(\jmb{h}^t_2, g_l(\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}))))
%\end{aligned}
%\end{equation}
%%\slwang{$f$ is not defined.}
%Here, we have presented skip functions in the decoder. 
%% For our stereo compression models, w
%We have similarly implemented skip functions in the encoder as well and found marginally better results. Our skip functions range from levels $l=1,2,3$, where $l=4$ represents the final reconstruction of the image $\hat{\jmb{x}}_1, \hat{\jmb{x}}_2$. Hence, the maximum height/width of $\jmb{h}^t_1$, $\jmb{h}^t_2$ used in $g_l$ is $H/2, W/2$. 
%
%In terms of the actual operations to predict $\jcb{\gamma}$ and $\jmb{S}^t$, we use convolutional layers + GroupNorm\cite{wu_groupnorm} + ReLU's as the building blocks for predicting and upsampling $\jcb{\gamma}(\bar{\jmb{y}}_1, t)$, concatenating $\jmb{h}^t_1, \jmb{h}^t_2, \jcb{\gamma}(\bar{\jmb{y}}_1, t)$, and predicting $\jmb{S}^t$. A general illustration is given in Fig. \ref{fig:stereo_complex_model} but more specific details are given in our supplementary material.
%%The context $\gamma$ is flexible. In our setting, we design $\gamma$ as  $\gamma(\bar{y_1}, l)$, a function of the first image code and the level. The output of $\gamma$ is an initial ``disparity volume" $S^{dinit}$ of dimensions $B \times C^{dinit} \times D \times H/16 \times W/16$. Our architecture consists of 3 levels of skip functions, and we ensure $C^{dinit}$ is divisble by 3: $S^{dinit}_{0:\frac{C^{dinit}}{3}}$ corresponds to $\gamma(\bar{y_1}, l=1)$, $S^{dinit}_{\frac{C^{dinit}}{3}:\frac{2C^{dinit}}{3}}$ corresponds to $\gamma(\bar{y_1}, l=2)$, etc. The intuition here is that different channel groups in $S^{dinit}$ correspond to different initial estimates of disparities at a given level. \slwang{rewrite this paragraph since it could be improved by a lot. Starts with intuition why you need a context and what could be encoded into a good context. Then what's the context module's arhictecture design. Some of the details could go to supp. Notations could be more clear.}
%%\jerry{Did an initial pass of adding intuition, not sure what could go into supp}
%We refer to our stereo model as the "Disparity Stereo Model", or DSM. 
